Aligning Non-Causal Factors for Transformer-Based Source-Free Domain Adaptation

Conventional domain adaptation algorithms aim to achieve better generalization by aligning only the task-discriminative causal factors between a source and target domain. However, we find that retaining the spurious correlation between causal and non-causal factors plays a vital role in bridging the domain gap and improving target adaptation. Therefore, we propose to build a framework that disentangles and supports causal factor alignment by aligning the non-causal factors first. We also investigate and find that the strong shape bias of vision transformers, coupled with its multi-head attention, make it a suitable architecture for realizing our proposed disentanglement. Hence, we propose to build a Causality-enforcing Source-Free Transformer framework (C-SFTrans) to achieve disentanglement via a novel two-stage alignment approach: a) non-causal factor alignment: non-causal factors are aligned using a style classification task which leads to an overall global alignment, b) task-discriminative causal factor alignment: causal factors are aligned via target adaptation. We are the first to investigate the role of vision transformers (ViTs) in a privacy-preserving source-free setting. Our approach achieves state-of-the-art results in several DA benchmarks.

==> round2_tables/algo.tex <==
\begin{algorithm}[!t]

\caption{DSiT Training Algorithm}
\label{algo:overall}
\begin{algorithmic}[1]
\vspace{1mm}
\Statex \underline{\textbf{Vendor-side training}}

\vspace{1mm}
\State \textbf{Input:} Let $\mathcal{D}_s$ be source data , $\mathcal{D}_{s}^{[i]}$ be augmented DRI dataset for each augmentation $\mathcal{A}_i$, ImageNet pretrained DeiT-B backbone $h$ from \cite{xu2021cdtrans}, randomly initialized goal classifier $f_g$ and randomly initialized domain classifier $f_d$.

\vspace{1mm}
\For{$iter < MaxIter$}:
\vspace{1mm}
\Statex \underline{{\textit{Goal task training}}}
\vspace{1mm}
\For{$iter < MaxTaskIters$}:
\State Sample batch from $\mathcal{D}_s$ 
\State Compute $\mathcal{L}_{cls}$ using Eq.\ 2 (main paper)
\State \textbf{update} $\theta_h\setminus\theta_Q, \theta_{f_g}$ by minimizing $\mathcal{L}_{cls}$
\EndFor

\vspace{1mm}
\Statex \underline{{\textit{Domain classifier training}}}
\vspace{1mm}
\For{$iter < MaxDomainIters$}:
\State Sample batch of DRI from $\mathcal{D}_{s}^{[i]}$
\State Compute $\mathcal{L}_{dom}$ using Eq.\ {1} (main paper)
\State \textbf{update} $\theta_{Q},\theta_{f_d}$ by minimizing $\mathcal{L}_{dom}$
\EndFor
\vspace{1mm}
\Statex \jnkc{\Comment{The two steps are carried out alternatively
}}
\EndFor

\vspace{1mm}
\Statex \underline{\textbf{Client-side training}}

\vspace{1mm}
\State \textbf{Input:} Target data $\mathcal{D}_t$, Target augmented DRI data $\mathcal{D}_t^{[i]}$, source-side pretrained backbone $h$, goal classifier $f_g$ and domain classifier $f_d$.

\vspace{1mm}
\For{$iter < MaxIter$}:
\vspace{1mm}
\Statex \underline{{\textit{Goal Task Training}}}
\vspace{1mm}
\For{$iter < MaxTaskIters$}:
\State Sample batch from $\mathcal{D}_t$
\State Compute $\mathcal{L}_{im}$ and $\mathcal{L}_{div}$ using Eq.\ \ref{sup:eqn:loss_im}, \ref{sup:eqn:loss_div} (suppl.)
\State \textbf{update} $\theta_h \setminus \theta_Q, \theta_{f_g}$ by minimizing $\mathcal{L}_{im} + \mathcal{L}_{div}$
\EndFor

\vspace{1mm}
\Statex \underline{{\textit{Domain classifier training}}}
\vspace{1mm}
\For{$iter < MaxDomainIters$}:
\State Sample batch of DRI from $\mathcal{D}_{t}^{[i]}$
\State Compute $\mathcal{L}_{dom}$ using Eq.\ {1} (main paper)
\State \textbf{update} $\theta_{Q},\theta_{f_d}$ by minimizing $\mathcal{L}_{dom}$
\EndFor
\vspace{1mm}
\Statex \jnkc{\Comment{The two steps are carried out alternatively.
}}

\EndFor

\end{algorithmic}
\end{algorithm}

==> round2_tables/augs.tex <==
\begin{table}[h]
\vspace{-2mm}
\setlength{\tabcolsep}{8pt}
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}cccccc@{}}
    \toprule
    \textbf{No. of augs.} & \textbf{Ar $\shortrightarrow$ Cl} & \textbf{Cl $\shortrightarrow$ Pr} & \textbf{Pr $\shortrightarrow$ Rw} & \textbf{Rw $\shortrightarrow$ Ar} & \textbf{Avg.} \\ \midrule
    3 & 64.3 & 79.9 & 84.6 & 80.0 & 77.2 \\
    6 & 70.0 & 86.8 & 87.6 & 82.5 & 81.7 \\ \bottomrule
\end{tabular}}
\vspace{-3mm}
\end{table}

==> round2_tables/task_epochs.tex <==
\begin{table}[h]
    \vspace{-2mm}
    \centering
    \setlength{\tabcolsep}{7pt}
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{ccccccc}
            \toprule
             \textbf{TE} &
             \textbf{SE} &
             \textbf{Ar $\shortrightarrow$ Cl} & \textbf{Cl $\shortrightarrow$ Pr} & \textbf{Pr $\shortrightarrow$ Rw} & \textbf{Rw $\shortrightarrow$ Ar} & \textbf{Avg.} \\
            \midrule
            1 & 5 & 62.7 & 79.3 & 84.6 & 79.2 & 76.8 \\
            5 & 1 & 70.6 & 87.7 & 88.5 & 82.3 & 82.2 \\
            \bottomrule
        \end{tabular} 
        }
        \vspace{-3mm}
\end{table}
